PointHPS: Cascaded 3D Human Pose and Shape Estimation from Point Clouds

Human pose and shape estimation (HPS) has attracted increasing attention in recent years. While most existing studies focus on HPS from 2D images or videos with inherent depth ambiguity, there are surging need to investigate HPS from 3D point clouds as depth sensors have been frequently employed in commercial devices. However, real-world sensory 3D points are usually noisy and incomplete, and also human bodies could have different poses of high diversity. To tackle these challenges, we propose a principled framework, PointHPS, for accurate 3D HPS from point clouds captured in real-world settings, which iteratively refines point features through a cascaded architecture. Specifically, each stage of PointHPS performs a series of downsampling and upsampling operations to extract and collate both local and global cues, which are further enhanced by two novel modules: 1) Cross-stage Feature Fusion (CFF) for multi-scale feature propagation that allows information to flow effectively through the stages, and 2) Intermediate Feature Enhancement (IFE) for body-aware feature aggregation that improves feature quality after each stage. To facilitate a comprehensive study under various scenarios, we conduct our experiments on two large-scale benchmarks, comprising i) a dataset that features diverse subjects and actions captured by real commercial sensors in a laboratory environment, and ii) controlled synthetic data generated with realistic considerations such as clothed humans in crowded outdoor scenes. Extensive experiments demonstrate that PointHPS, with its powerful point feature extraction and processing scheme, outperforms State-of-the-Art methods by significant margins across the board. Homepage: https://caizhongang.github.io/projects/PointHPS/.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> figures/method_cff.tex <==
\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{images/method_cff.jpg}
  \setlength{\abovecaptionskip}{0cm}
  % \vspace{-5mm}
  \caption{Cross-stage Feature Fusion (CFF). We empirically find that CFF is critical to an effective cascade of feature extraction stages as information could be lost in the iterative downsampling and upsampling phases. }
  \label{fig:method_cff}
\end{figure}

==> figures/method_ife.tex <==
\begin{figure}[]
  \centering
  % \vspace{-5mm}
  \includegraphics[width=\linewidth]{images/method_ife.jpg}
  \setlength{\abovecaptionskip}{0cm}
  \vspace{-5mm}
  \caption{Intermediate Feature Enhancement (IFE). Joints regressed from the coarse SMPL estimation are used as center or anchor points. Ball query and grouping are performed to aggregate neighboring point features into joint features. Hence, with body structure implicitly encoded, the joint features are used to enhance point features through Efficient Attention. We highlight that the coarse SMPL estimation might not be perfect but through iterative IFE in the cascaded architecture, significant improvements are achieved.}
  \label{fig:method_ife}
\end{figure}

==> figures/multistage.tex <==

\begin{figure}[]
  \centering
  \vspace{-5mm}
  \includegraphics[width=0.85\linewidth]{images/multistage.jpg}
  \setlength{\abovecaptionskip}{0cm}
  \caption{From HMR3D to \name. a) HMR3D is an extension of HMR from 2D input to 3D input (\Sec\ref{sec:method:hmr3d}) that performs surprisingly well on real-captured point clouds. b) We design \name to have multiple stages of a HMR3D-like structure to iteratively refine the estimation. A more elaborate illustration of the stage is shown in \Fig\ref{fig:method}, including IFE and CFF (indicated by blue arrows) modules.}
  \label{fig:multistage}
\end{figure}

==> figures/pve_vs_visibility.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/pve_vs_visibility.jpg}
  \setlength{\abovecaptionskip}{0mm}
  \caption{Box plot of PVE under various extent of occlusion. The orange line indicate median, the box indicate the range between the lower and the upper quartiles, and the whiskers indicate the range of the results. Examples with fewer than three visible parts are very rare, and are excluded due to the lack of statistical significance.}
  \label{fig:pve_vs_visibility}
\end{figure}

==> figures/real_vs_synthetic.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/real_vs_synthetic.jpg}
  \setlength{\abovecaptionskip}{0cm}
  \vspace{-2mm}
  \caption{An analysis on the differences between real and existing synthetic data. In b), we sample 1,000 sequences from each dataset and plot the mean distance from a point to the nearest SMPL vertex and observe a significant gap. Points from a) HuMMan are often some distances away from the underlying human geometry whereas points from c) SURREAL are sampled on the surface of the SMPL annotation. }
  \label{fig:real_vs_synthetic}
\end{figure}

==> figures/visual_gta_selected.tex <==
\begin{figure}[t]
  \centering
  % \vspace{-2mm}
  \includegraphics[width=0.95\linewidth]{images/visual_gta_selected.jpg}
  \setlength{\abovecaptionskip}{0cm}
  \caption{Visualization of \name's performance on GTA-Human++. We show the estimation results of the subject in the red bounding boxes.  GTA-Human++ includes challenging scenes with occulusion-induced incomplete point clouds. The point cloud may be drawn from a different angle for better visualization than the original virtual camera.}
  \label{fig:visual_gta_selected}
\end{figure}

==> figures/votehmr_seg.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{images/votehmr_seg.jpg}
  \setlength{\abovecaptionskip}{0cm}
  \vspace{-2mm}
  \caption{Body part segmentation results of VoteHMR. a) color map for 24 body parts. We observe that VoteHMR does not produce satisfactory part segmentation results, which is a critical auxiliary task in its pipeline. b) and c) show two examples where the left point cloud is the estimated part results by VoteHMR~\cite{liu2021votehmr} whereas the right is the ground truth.}
  \label{fig:votehmr_seg}
\end{figure}
